Classical Amplitudes in Gravitational-Wave Physics

In this thesis, we study emission amplitudes for the class of nonlinear processes of tails, which are processes of order $G_N^2$, and represent the effect of scattering gravitational radiation off the static background curvature, including not only mass tails but also the "failed" tails due to the angular momentum of the source. As originally shown in our work, some of these amplitudes present anomalies, which are then properly understood and corrected with field theory tools which have straightforward counterpart in traditional methods. We also investigate the relation between emission and self-energy diagrams and, in particular, show that a correction to the anomalous self-energy diagrams is necessary to correctly account for conservative terms that arise from radiative processes. From this, we obtain the correct contribution to the conservative 5PN stemming from the electric quadrupole angular momentum failed tail, correcting previous results in the literature. Besides this, we also compute for the first time the conservative contributions from the angular momentum failed tail, for arbitrary multipole moments. Subsequently, we explore the natural higher-order extension (of order $G_N^3$) of the mass tails, called tails of tails, for generic electric and magnetic multipoles. As we will see, both long- and short-distance divergences are encountered, which are then properly understood and dealt with in terms of standard renormalization techniques. In this case, we are able to resum the logarithmic contributions through the integration of the renormalization group equation. Thus, in this thesis, we have extended the post-Newtonian perturbative expansion in the particularly thorny region of processes involving the mixture of radiative and potential modes.

==> chapter0/introduction__old_.tex <==
\chapter{Introduction}

The starting point of our discussion is the general theory of relativity. As it is more commonly known, general relativity is the theory of space, time, and gravitation formulated by Albert Einstein in 1915, originally devised in a series of four papers \textcolor{red}{\cite{Einstein1915a,Einstein1915b,Einstein1915c,Einstein1915d}}. In 1916, soon after the establishment of his relativistic version of a theory of gravity, Einstein realized that his field equations, when considered a weak-field regime, had wave solutions \textcolor{red}{\cite{Einstein1916}}. These waves, called \texttt{gravitational waves}, are transverse perturbations traveling across spacetime at the speed of light, generated by time variations of the mass quadrupole moment of the source \textcolor{red}{\cite{Einstein1918}}.


Nevertheless, direct observation of gravitational waves were only accomplished nearly a century after Einstein predicted their existence: On September 14, 2015, the two detectors of the Laser Interferometer Gravitational-Wave Observatory (LIGO) \textcolor{red}{\cite{LIGO2015}} simultaneously detected a transient gravitational-wave signal \cite{LIGO2016a}. 
This signal, soon after confirmed to correspond to gravitational waves emitted from the coalescence of a binary black hole (BBH) system, was dubbed GW150914\footnote{Gravitational-wave signals are named after the date of their discovery. In this case, \textit{e.g.}, the signal detected in 2015-09-14 goes by the name of GW150914.} and represented the first of many gravitational-wave events of astrophysical origin that would later be observed. The importance of GW150914 goes beyond this and also relies on the fact that it demonstrated %confirmed 
the existence of %such astrophysical configuration 
binary stellar-mass black hole systems
and provided the first observed BBH merger. With this, a new observation window was opened, setting the beginning of the field of gravitational-wave astronomy \cite{CERNCourier}.

In the three months following the first detection, the two LIGO detectors observed two other gravitational-wave events: GW151012 and GW151226 \textcolor{red}{\cite{LIGO2016b,LIGO2016c}}. Like in GW150914, these two signals were produced during the coalescence of binary systems of stellar-mass black holes. The three events GW150914, GW151012, and GW151226 were the only ones observed during the first run of observation (O1) of Advanced LIGO, which took place from the 12th of September, 2015, to the 19th of January, 2016. Then, after an upgrade and commissioning period, the second observing run (O2) started on the 30th of November, 2016. On August 1, 2017, Advanced Virgo \textcolor{red}{\cite{Virgo2015}} joined the twin LIGO detectors, with this newly-formed network of advanced interferometers having observed a total of eight events by the end of O2, on August 25 of the same year
\textcolor{red}{\cite{LIGO2017a,LIGO2017b,LIGO2017c,LIGO2017d,LIGO2019}}. 
Among these events, seven corresponded to stellar-mass BBHs, while one, GW170817, was identified to have originated from a binary neutron star (BNS) inspiral \textcolor{red}{\cite{LIGO2017d}} in a joint detection of gravitational waves along with an electromagnetic counterpart \textcolor{red}{\cite{GWeEM1,GWeEM2}}. This later fact makes GW170817 a unique event, important in this era of multimessenger astronomy opened by gravitational-wave observations. 
%%%% unique
For a detailed account on the astrophysical properties of the events comprising the first and second runs of the LIGO-Virgo detector network, the reader is referred to the first Gravitational-Wave Transient Catalog (GWTC-1) in Ref. \cite{LIGO2019}.

Although GW170817 was the first BNS gravitational-wave signal to be \textit{directly} detected, it is not, however, the first time a BNS system was observed: in 1974, Russell Hulse and Joseph Taylor discovered a binary system formed by two pulsars (i.e., rapidly spinning neutron stars), called PSR B1913+16, and also known as the Hulse-Taylor pulsar \textcolor{red}{\cite{HulseTaylor1975,Hulse1994}}. This binary system is historically important since later on, in 1981, Taylor, along with Joel Weisberg, observed the effect of energy loss due to the emission of gravitational radiation on the orbit of this system, indirectly proving the existence of gravitational waves \textcolor{red}{\cite{TaylorWeisberg1975}}.

The third and most recent observing run, O3, took place during the years of 2019 and 2020, and was split into two parts, O3a and O3b. In the first half of this observing run, O3a, with data taken from 1 April to 1 October, 2019, Advanced LIGO and Advanced Virgo were able to observe 44 new gravitational-wave binary coalescences. Such observations comprised 42 BBHs, 1 BNS and one binary system containing a black hole and a compact object whose nature could not be discerned, GW190814, being either the lightest black hole or the heaviest neutron star ever known \cite{LIGO2020}. In addition to this interesting signal, O3a counted also with 
GW190412, the first BBH observation with asymmetric constituent masses ($m_1=30.1 M_{\odot}, m_2 = 8.3M_{\odot}$)  \cite{LIGO2021}, although GW190814 would later turn out to be even more asymmetric, with individual masses of $ 23M_{\odot}$ and $2.6M_{\odot}$; 
GW190425, the second gravitational-wave event consistent with a BNS coalescence \cite{LIGO2021};
and GW190521, a BBH merger with total final mass of $\sim 150M_{\odot}$, being the heaviest final stage stellar black hole to be observed by the LIGO-Virgo Collaboration \cite{LIGO2020a,LIGO2020b}. Details can be found in \cite{GWTC2,GWTC21}, in the second catalog GWTC-2 and the extended GWTC-2.1.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The second half of the third observing run, O3b, operated from 1 November, 2019, to 27 March, 2020, and added 35 new events to the previous observing runs. Among these signals, 3 corresponded to the first confident detections of neutron star-black hole (NSBH) coalescences, while the other 32 stemmed from BBH mergers. No BNS events were observed during O3b. For a complete analysis and details of the astrophysical properties of these detections, please check the third Gravitational-Wave Transient Catalog GWTC-3 out in Ref.~\cite{GWTC3}. With this, a total of 90 gravitational-wave signals from binary system coalescences  have been detected since the beginning of the first observing run in 2015. See Table~\ref{GWTCevents} for a brief summary of the three observing runs.
\begin{table}
\centering
\begin{tabular}{c|c|c|c}
\hline
Observing run & Number of events & Start date & End date\\ 
\hline
O1 & 3 BBH & 12-Sep-2015 & 19-Jan-2016 \\
O2 & 8 = 1 BNS + 7 BBH & 30-Nov-2016 & 25-Aug-2017 \\
O3a & 44 = 1 BNS + 42 BBH + 1(?) & 1-Apr-2019 & 1-Oct-2019 \\
O3b & 35 = 32 BBH + 3 NSBH & 1-Nov-2019 & 27-Mar-2020 \\
\hline
\end{tabular}
\caption{Summary of the LIGO-Virgo  observing runs, BBH, BNS, and NSBH standing respectively for binary black hole, neutron star, and neutron star-black hole  mergers. The question mark in O3a corresponds to GW190814, which is either a BBH or NSBH merger.}
\label{GWTCevents}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\textcolor{red}{The next observing run, O4, is planned to start in March 2023}, with the two LIGO and the Virgo detectors being joined by the Japanese interferometer KAGRA \cite{KAGRA} in the newly formed LIGO-Virgo-KAGRA (LVK) collaboration.
The prospects for the near future are that the new upgrades will allow us to increase considerably the number of detections as well as will allow us to see much farther, into cosmological scales. This progress calls for an immediate effort towards improving the precision of the templates currently used by the LIGO-Virgo-KAGRA collaboration. In particular, the current models of gravitational-wave templates used in these detections are especially sensitive to the phase of the gravitational wave (GW), which has to be modeled very precisely in order to lead to reliable interpretation of the data. 
This phase, $\Phi(t)$, which tracks the orbital phase evolution of compact binary systems, is given in terms of the conservative energy of the system, $E$, as well as in terms of the radiated power loss due to gravitational radiation, $P$, through
%%%%%%%HERE HERE HERE HERE HERE
\begin{equation}
    \Phi(t) = 2 \int^t_{t_0} dt\, \omega(t) = - \frac{2}{G_N M} \int^{v(t)}_{v(t_0)}dv \frac{v^3}{P(v)}\frac{dE}{dv}\,.
\end{equation}
In this expression, $\omega(t)$ is the orbital phase of the binary system's motion, and $t_0$ and $t$ respectively the time where
the signal enters and exits the detector. 

In modelling the phase as above, it is assumed that the system goes through an adiabatic inspiral phase, going through a succession of quasi-circular orbits, inspiralling inward, and driven by gravitational-radiation reaction. In fact, this provides a very good approximation, that optimizes the analysis of the gravitational-wave data, since it is well known that, for typical compact binary systems observed by interferometers like LIGO, by the time when the gravitational wave enters the bandwidth of the detectors, their orbits will have already been circularized long before due to the radiation reaction on the initially elliptic orbits \textcolor{red}{REFXX}.
This is achieved upon the fundamental assumption that the system's energy loss is solely due to the emisson of gravitational radiation, through the energy balance equation
\begin{equation}
\frac{dE}{dt} = - P\,.
\end{equation}  



The two quantities needed to construct the gravitational-wave phase, the conserved energy and the energy flux are appropriately modeled within the post-Newtonian approximation to general relativity. In this formalism, the Einstein field equations are solved perturbatively, iterating sucessive orders in powers of $v^2$, the relative velocity square, which serves as the small parameter of the expansion, and accounts for deviation of the slow-motion and weak-field regime, characteristic of linearized gravity. The most important application of this formalism is in describing the coalescence of compact binary systems, extending the Newtonian results to incorporate fast-motion and strong-field contributions as predicted by general relativity. This is essential in the construction of templates currently under use by laser-interferometric observatories to detect gravitational-wave signals emitted by inspiraling  binaries. For the most complete and up-to-date review on the post-Newtonian formalism, and in particular, applied to problem of inspiralling compact binaries, from traditional methods, see Ref.~\cite{blanchetlivrev}.

In the post-Newtonian approximation, the $n$th correction $(v^2)^n$ beyond the Newtonian expression is said to be the $n$PN order. Hence, considering the motion of two spinless particles, the 1PN correction was first derived by Lorentz and Droste \textcolor{red}{\cite{lorentz1917a,lorentz1917b}}, and later on confirmed by Einstein, Infeld and Hoffmann in \textcolor{red}{Ref.~\cite{EIHlagrangian}}, where the 1PN for the general $N$-body system was obtained. The 2.5PN equations of motion, which includes the first appearance of radiation-reaction effects, was later on derived by Damour and Deruelly \textcolor{red}{\cite{damour1981,damour1983}} using a post-Minkowskian approach. The 2.5PN order for the equations of motion was also obtained by Schäfer in Ref.~\textcolor{red}{\cite{schafer1985}} from an ADM Hamiltonian approach and within the post-Newtonian iteration of the Einstein field equations by Blanchet, Faye and Ponsot \textcolor{red}{\cite{blanchet1998}}. The 3PN \textcolor{red}{equations of motion} were first obtained in REF \textcolor{blue}{[6-8]} using the ADM formulation of general relativity, and \cite{blanchet2000,blanchet2001} \textcolor{blue}{[10-11]} in harmonic coordinates from traditional methods, with equivalent results \textcolor{red}{\cite{andrade2001,damour2001}}. The equations of motion at the 4PN order was also obtained by different groups, including Ref.\textcolor{red}{~\cite{damour2014}}, derived within the ADM formulation, and Ref.\textcolor{red}{~\cite{bernard2016}}, from traditional post-Newtonian methods. \textcolor{red}{Nevertheless, the two results differ by a local term.} \textcolor{red}{This has mostly centain been solved by now (see RSSF 4PN and blumlein.)}







The state-of-the-art of the gravitational-wave phase currently used in LVK's pipelines is the 3.5PN order, and was first obtained in Ref.~\cite{blanchet2005a}, with the energy $E$ computed in \cite{blanchet2000,blanchet2001}, (Because no corrections to the energy are present at the 3.5PN order, the 3PN expression is also valid through the 3.5PN order.) although with some free, undetermined parameters due to the incompleteness of the regularization technique used there, the Hadamard one, and completed in Ref.~\cite{blanchet2004} with the aid of dimensional regularization. In Ref.~\cite{blanchet2005a}, besides the energy to the 3.5PN order, it was also required the emitted power loss at the same order\footnote{For the gravitational radiation field, and related observables, the post-Newtonian corrections are considered beyond the quadrupole formula. In this case, e.g., the 1PN correction to the energy flux is the 1PN relative order beyond the leading-order computed from the quadrupole in the Newtonian orbit.}, previously obtained in Refs.~\textcolor{blue}{[18,13]} using the so-called wave-generation formalism \textcolor{blue}{[12-14]}. In this formalism, that describes the exterior gravitational field to the composite system, and is based on a post-Minkowskian approximation, an expansion in powers of $G_N$, the source degrees of freedom are parametrized by a series of multipole moments, and observables at infinity are given in terms of nonlinear relations involving such quantities. Afterwards, this multipole moments can be matched in the region close the sourse, to be given in terms of the orbital variables of the binary system within the post-Newtonian approximation.  


\vspace{1cm}

Spin effects can also be incorporated to the orbital phase evolution of the system, and are known up to the 2.5PN order \textcolor{blue}{[5]}.

\textcolor{gray}{Currently, we know the complete templates up to the 2.5PN order [24-26]" Refs from \cite{blanchet2000}}

Once the phase is obtained and templates of gravitational waves are built, spanning a large region in the parameter space of the binary \textcolor{red}{(these are the following 15 parameters:)}, we can start seeking for gravitational-wave signals. The usual technique employed in this case is the so-called matched filtering, which consists in correlating the detector's output to waveforms present in a template bank, and weighted over the characteristic noise of the detector. Hence, whenever a signal is detected and a correlation with a template of the bank is established, an spike emerges in the plot of this correlation, which then allow us to extract the signal within the noise. \textcolor{red}{Show original plot in the PRL of the first detection.} An interesting review on how precisely the output of the LIGO-Virgo detectors is analyzed, and gravitational-wave signals are extracted, can be foudn in \textcolor{red}{XXX}. 

In particular, the process of detecting gravitational waves from merging binary systems with laser interferometers that rely on the matched filtering requires accurate prediction for the gravitational waveform. In fact, a series of analysis performed in Refs.~\textcolor{blue}{[1-3]} have shown that the 3PN, or better the 3.5PN order provides a lower-bound accuracy below which the errors are too large to provide reliable interpretation of the detector's data. At the 3.5PN, on the other hand, we have a sufficiently accurate prediction for the waveforms, so that the errors are not too significant on the parameter estimation. Besides this, higher post-Newtonian orders are important to resolve and analyze signals coming from farther distances. This justify the need in attaining higher-order corrections to the equations of the motion and the radiation field in the post-Newtonian approximation, since the main goal lies in extracting reliable predictions of the theory that can be compared against the output of the detectors.


\vspace{1cm}

\textcolor{blue}{blue = REFs of \cite{blanchet2005a}}

\vspace{2cm}


In addition to the inspiral phase, that is fully described by the post-Newtonian formalism, the evolution of a compact binary system undergoes two other phases: the merger, when the two objects can no longer be resolved into two, but one single object, and the ringdown, when the two objects have given rise, typically, to a final stage black hole, which still oscillates as quasi-normal modes.  


``The resulting system, typically a BH finally settles down to its ground state, rediating away energy stored in its excited modes. This is the so-called `ringdown phase'".


\subsubsection{The phases of the coalescence}

\textcolor{red}{``Numerical relativity or approaches such as [4] (or \cite{blanchet2005}) could describe the plunge and merger phases. The latter approach starts from the PN expansion and goes beyond the adiabatic approximation."} Pages 28 and 29 of Alessandra's notes.

\textcolor{gray}{``When the two compact objects approach each other towarde merger, the PN expansion will lose accuracy and should be taken over by numerical-relativity computatoins [359,116,21]", ``Despite very intensive developments of numerical relativity, the PN approximation remains indispensable for describing the inspiral phase of compact binaries to high accuracy, and for providing a powerful benchmark against which the numerical computations are tested."} Living review of Luc, page 8.

\textcolor{blue}{For reviews on BH perturbation and the self-force approach see Refs. [348, 373, 177, 23]}. From review by Luc.

\textcolor{red}{Falar brevemente do EOB.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newpage

\subsubsection{The effective field theory for gravity}


Although the origin of Post-Newtonian methods dates back to the \textcolor{red}{early} 1920s, following the early days of General Relativity itself,  only in the last two decades that this approximation method gained a field-theoretical format. 
To be more precise, in a 2006 paper \cite{rothstein2006}, I. Rothstein and W. Goldberger formulated an effective field theory (EFT) to describe the dynamics of two compact objects, completely compatible with the Post-Newtonian approximation. This EFT was then coined Non-Relativistic General Relativity (NRGR) as a parallel to NRQCD, which serves as the basis for the construction. Since then, this formulation has attracted a lot of attention from until then disconnected communities: on one side, relativists interested in the classical aspects of gravity, on the other, theorists  interested in practical applications of the most recent tools of the ever-growing field of scattering amplitudes. This synergy has  great potential, being one of the most active research fields in physics nowadays. 

To list a few of the most prominent features of this EFT implementation of the Post-Newtonian approximation, we have (1) it gives separate descriptions for the conservative and dissipative dynamics of the binary system, (2) it provides a clear power counting from which the perturbative approach is implemented, in which case Feynman diagrams are used to ease the tracking of contributions, besides easily incorporating (3) nonlinearities stemming from general relativity, (4) spin effects, and even (5) modifications to general relativity. Additionally, (6) it also provides a better understanding of the UV and IR divergences present in the theory in light of the (classical) renormalization group evolution. 

As it soon becomes clear, the number of Feynman diagrams involved in each step increases enormously as we seek for higher and higher orders, and methods of the field of scattering amplitudes have to be considered in order to gain efficiency in computing higher-order effects. In particular, the state-of-the-art description of the conservative dynamics of binary systems lies in the 4PN order \cite{RSSF4PNa,RSSF4PNb}, i.e., fourth-order in $v^2$ beyond the Newtonian solution, in which case the binary constituents can still be described by point particles.  This is the order in which radiation-reaction terms start to contribute \cite{RSSFhereditary}. Radiation reactions are effects present in the interplay of different scales, between the so-called potential and radiation modes, with the corresponding imprint to the two-body potential having already been completely accounted for, and the pair of IR-UV divergences, present in the different regions, being mutually canceled and duly understood \cite{RSSF4PNb}.    

\textcolor{gray}{Within this effective-field-theory framework, the 3PN Lagrangian in harmonic coordinates was first derived in \textcolor{red}{Ref.~\cite{RSSF2011}}. Mention spin here!}

Advances towards the complete understanding of the 5PN order represent currently the most important problem within the relativistic two-body problem. This is, in particular, the order in which finite-size effects start to appear \cite{rothstein2006} and, therefore, that allow us to probe the strong-field regime of gravity via gravitational waves, and expected to finally provide insights towards the problem of the equation of state for neutron stars. At this order, despite the purely conservative description having already been computed for the spinless case \cite{blumlein2021}, and not introducing any further conceptual obstacle, radiation-reaction effects pose a notoriously tough and challenging problem. As a matter of fact, current results of 5PN radiation-reaction contributions to the binary system dynamics is in conflict with information stemming from self-force and \textit{Tutti-Fruti} calculations, as pointed out last year by D. Bini, T. Damour, and A. Geralico \cite{damour2021}. 
Among the novelties at this order, there is the inclusion of higher-order terms of a particular type of radiation-reaction effect called “hereditary” \textcolor{red}{REFXX}. These are effects entering the two-body dynamics in a nonlocal fashion, depending on the history rather than on the instantaneous state of the source at retarded time. Particular examples of such a class of phenomena are the tail and memory effects, whose contribution to the conservative sector involves a cubic multipole moment interaction. In particular, for the 5PN order, we must include higher-order tail effects for the electric quadrupole and octupole moments and magnetic quadrupole, the quadrupolar angular-momentum tail-like contribution, as well as the nontrivial quadrupole memory. All these processes affect the two-body dynamics inasmuch as nonlinear interactions induce gravitational radiation to back-scatter \cite{RSSFhereditary}.



%The resolution to this difficult problem relies upon investigating different aspects of the interaction between higher-order radiation-reaction effects and observables from gravitational-wave emission amplitudes, as well as studying the interplay between the potential and radiation zones in the interface in which they overlap. To be more precise, one needs to (i) understand how to consistently separate conservative and dissipative contributions from the aforementioned nonlinear effects; (ii) Compute the corresponding waveforms, so one can, afterward, directly compute observables such as the emitted power and angular momentum loss, serving as a consistency check for the results of the previous item, as well as to provide a better interpretation of the physics involved; And finally, (iii) compute these same radiation-reaction effects directly in terms of the orbital variables, therefore explicitly deriving the complete conservative dynamics, which will then include long-distance logarithms, intending to check the explicit cancellation of UV/IR poles from the different scales involved, as already successfully done at the 4PN order.



\vspace{1cm}


At the 5PN order,  there are important physical effects that also start to contribute at this order, namely the memory effect and other higher-order tail contribution beyond the leading electric quadrupole case. In particular, since these higher-order dissipative effects are highly non-trivial in nature, one has to be very careful on how to treat such time-asymmetric phenomena at the level of a path integral formulation.          



In this case, one has to resort to the so-called \textit{in-in} formalism, also known as the \textit{closed time path} formalism \cite{schwinger61,keldysh65}. The in-in formalism is a field-theory formulation that appropriately incorporates causal interactions associated with nonconservative processes, like radiation-reaction, at the level of path integral and Feynman diagrams. Applications to our setup have already been done in the study of leading radiation-reaction effects \cite{galleytiglio}, as well as in the leading hereditary contribution \cite{GalleyRoss2016}, namely the tail. Nevertheless, higher-order hereditary effects entering the 5PN conservative dynamics, like the memory, are more involved and have never been fully explored. A proper investigation needs to be carried out.

Another approach that has recently been pursued to study the relativistic two-body problem is an EFT implementation of the post-Minkowskian approximation (PM) \cite{zvi2019}, which has essentially Newton's constant as the appropriate parameter of the expansion, as a weak-field regime approximation. In this formulation, rather than a bound system, the focus is on the scattering of two compact objects, with the scattering angle as the most important observable to be computed. This is, in particular, a complementary and powerful gauge-invariant way of studying radiative corrections to the conservative dynamics of binary systems, being also very important for providing independent checks of results obtained via NRGR calculations \cite{damour2021}. A thorough investigation of higher-order hereditary effects, both from the use of the in-in formalism in the context of NRGR and from the study of the scattering angle in the PM approximation (in which the in-in formalism continues to be important), considering in particular the memory interaction, is the main path we are currently investigating.







\vspace{2cm}


\textcolor{blue}{\textbf{The outline} of this ``Pre-Thesis" is the following: In Chap.~2, we review the basic theory of gravitational waves following from the linearized theory of general relavitity. This will serve as basis for subsequent chapters. In Chap.~3, we review the relativistic two-body problem from an effective field theory (EFT) perspective. In this chapter, the basic construction of the EFTs is introduced based on the separation of scales present in the theory and basic computation of Feynman diagrams is performed. Chap.~4 is devoted to present original research: in this chapter, we study the classical renormalization of the whole series of multipole moments present at the far zone EFT, i.e., the effective theory that describes gravitational radiation. In this work, both infrared and ultraviolet divergences are encountered, and knowing how to deal with them is essential to understand the mixing of scales present at the conservative and dissipative sectors of the theory.
Finally, in Chap.~5, we present the perspectives and project schedule to tackling the most important problem: the inclusion of radiation-reaction effects to the conservative dynamics of the two-body system. }





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage


\section{Perspectives}

In the first of these papers, namely the one with title ``Classical Gravitational Self-Energy from Double Copy", we investigate the possibility of relating gravity self-energy amplitudes computed in the far zone to some sort of ``square" of non-Abelian gauge field theory amplitudes of the same type, using the so-called \textit{double-copy} rules. To this end, an analogue multipole moment effective action is build on the gauge side, which now describes how the color charged source couples to the non-Abelian gauge field. On the gravity side, besides the spin-2 tensor field, there are also other degrees of freedom: a dilaton, and an axion, that compensate the four degrees of freedom present on the \textit{double-copied} gauge theory side. An explicit duality is built for the non-trivial self-energy diagrams corresponding to the tail process, to all multipole moments.    

In the third paper, ``Tail contributions to gravitational conservative dynamics", we compute tail contributions to the conservative dynamics of a generic self-gravitating system,  for every multipole order, of either electric and magnetic parity. Such contributions arise when gravitational radiation is backscattered by the static curvature generated by the source itself and reabsorbed. Tail processes are relevant for the study of compact binary dynamics starting from the fourth post-Newtonian order. Within this context, we resolve a discrepancy recently arised at fifth post-Newtonian order between effective field theory and self-force results.



==> rest/rest.tex <==
\chapter{rest}


\section{Notes for GWs chapter}


\newpage


\vspace{2cm}
\textbf{References followed so far in this chapter:}
\begin{itemize}
    \item M. Maggiore's book (vol.1) \cite{maggiore1}: Pages 1-40, 101-139. I skipped subsection ``Gravitational radiation and the equivalence principle" page 120. 
    \item A. Buonanno's 2007 review \cite{buonanno07}: Pages 7-18. 
\end{itemize}

\vspace{2cm}
\textbf{Possibly important ``Further reading" by Maggiore from Chapter 3}
\begin{itemize}
    \item \textbf{Quadrupole radiation:} Weinberg (1972)\\
          MTW (1973)\\
          Landau \& Lifshitz (1979), Vol. II.\\
          Straumann (2004): \textit{General Relativity. With Applications to Astrophysics.} \\
          Schutz \& Ricci (2001) (modern physical interpretation): In \textit{Gravitational Waves}, I. Ciufolini et al. eds, IoP Publishing, Bristol. 
    \item \textbf{GW generation:} Weinberg (1972), Section 10.4.\\
          Thorne (1983) (review): In \textit{Gravitational Radiation}, N. Deruelly and T. Piran eds., Les Houches 1982, North-Holland, Amsterdam.\\
          Thorne (1987) (review): In \textit{300 Years of Gravitation}, S. Hawking and W. Israel eds., Cambridge University Press, Cambridge.
    \item \textbf{Multipole expansion}: Thorne (1980): Rev. Mod. Phys. 52, 299.\\
          Damour \& Iyer (1991a): Phys. Rev. D 43, 3259.\\
\end{itemize}

\textcolor{red}{See Further reading of Chapter 5, page 299, of Maggiore's book. In particular, see papers with explicit formulas for the phase and waveform of a compact binary system. See also paper where the spin is included.}


Para o capítulo do básico de GWs, ler:
\begin{itemize}
\item 1. capítulo de Brunello
\item 2. capítulo de François
\item 3. Buonanno
\item 4. Refs. de Buonanno
\item 5. Slides de Buonanno from IHP school
\end{itemize}








\section{Notes from EFT chapter}


\newpage

\textcolor{red}{Comment on spins}


\textcolor{red}{From the review by Luc, page 9: ``The main problema with this approximation (PN), is its domain of validity, which is limited to the near zone of the source - the region surrounding the source that is of small extent with respect to the wavelength of the GWs", ``The PM expansion, by contrast, is uniformly valid, as soon as the source is weakly self-gravitating, over all spacetime."}

\textcolor{blue}{VERY IMPORTANT REF for the far zone: Thorne, K. S., ``The multipole moments have been extensively studied in the linearized theory, which ignores the gravitational forces inside the source" (page 10) - Multipole expansions of gravitational radiation”, Rev. Mod. Phys., 52, 299–339 (1980). [DOI], [ADS].}

\textcolor{red}{Still the Review by Luc, page 10: ``The general structure of the infinite multipole series in the linearized theory was investigated by several works [369, 367, 343, 403], from which it emerged that the expansion is characterized by two and only two sets of moments: massa-type and currecnt-type moments."}

\textcolor{gray}{Luc review, page 10: ``An alternative way of defining the multipole expansion within the complete non-linear theory is that of Blanchet and Demous [57, 41]. In this approach, the basic mlutipole moments are the \textit{source} moments, rather than the radiative ones. In a first stage, the moments are left unspecified, as being some arbitrary functions of time, supposed to describe and actual physics source.  They are iterated by means of a PM expansion of the vacuum field equation.", ``In this `multipolar-PM' formalism, which is physically valid over the entire weak-field region outside the source, and in particular in the wave zone, the radiative multipol moments are obtained in the forma of some non-linear functionals of the more baisc source moments."}

\textcolor{red}{Luc review, page 11: ``The domain of validity of the PN iteration (viz. the near zone) overlaps the exterior weak-field region, so that there exists an intermediate zone in which the PN and multipolar expansions can be matched together. This is ta standar application of the method of matched asymptotic expansions in GR [114, 113, 7, 357]"}

\textcolor{brown}{Luc review, page 11, valid for next chap as well: ``Matching the exterior multipolar and PM field to the PN source ir able to take into account any PN correction to both theh source and radiative mlultiople moments. The relationshops between the radiative and soruce moments include many nonlinear multipole interactoins, because the srouce moments mix with each other as they `propagate' from the source to the detector."}

\textcolor{blue}{Important refs on the tail, for the followins two chapters: [58, 43, 47] (refs form Luc's review). Other Refs important for the far zone: [57,41,44,49]}

\textcolor{red}{Radiation-reaction forces (ref from Luc's review) [114,113,319]. Refs for the 2.5PN RR force.}

\textcolor{blue}{Refs from Luc's review that might be interesting (not necessary though), about the Hulse-Taylor pulsar: [398,399,400]}

\textcolor{red}{On the effacemente principle: page 16 of Luc's review, Ref. [142] there (Damour).}

\textcolor{gray}{See point 3 in page 25 of Luc's review, on the method of matched asymptotic expansions.}

\textcolor{gray}{On the combination of the PM expansion and the multipolar expansion: page 26 of Luc's review, paragraph below Eqs. (33).}

\textcolor{gray}{On the constancy of the M (ADM), etc: page 27 of Luc's review, below Theorem 1.}

\textcolor{red}{ADD refs. especially in the ``method of regions" section.}

\textcolor{red}{Images in the correct latex environment.}

\textcolor{blue}{For the following chapter on GWs in the far zone, see bottom of page 30 in Luc's review, about the choice for the correcting term.}

\textcolor{gray}{For the following chapter, read again chapter 2 of Luc's review: too many important things. In particular, around page 31.}

\textcolor{gray}{For next chapter: [57] of Luc's review -> Blanchet and Damour on the proove that Eq. (49) is the most general solution of the vacuum equation.}

\textcolor{red}{Above Eq. (4.5) Maybe talk about the scalling of the Wilson coefficients.}
\textcolor{red}{For the present chapter: Paragraph starting with ``The sis sets", page 32 of Luc's, on the solution in terms of only two sets of multipoles moments. Read whole page!}

\textcolor{red}{Paper by Thorne, Ref [403] in Luc's review}

\textcolor{purple}{Other very important refs. [48,58, 42,50,60]}

\textcolor{blue}{Discuss about radiative moments and write general formulas for energy flux and angular momentum flux, Eqs.(68a) and (68b) in Luc's review.}

\textcolor{purple}{Sec. 3.2 of Luc's review: all about tails. Re-read this section for comments here on the INTRO and for later chapters.}


==> review/review.tex <==
\chapter{REVIEW AND CORRECTIONS}

\subsection{Important points to be used in the review of these writings:}
\begin{enumerate}
    \item \textcolor{red}{After finishing the writing of the first chapter, review notebook with Dino in the cover to check If I missed anything.}
    \item \textcolor{red}{See Refs by Alessandra Buonanno from the slides of the IHP School on GWs}
    \item \textcolor{red}{add the additional ref for the SVT decomposition from a cosmology paper}
    \item \textcolor{red}{notice or note?}
    \item \textcolor{red}{i.e., in italic or not?}
    \item \textcolor{red}{remove numbers in eqs not referred?}
    \item \textcolor{red}{In bolfdace or italic?}
    \item \textcolor{red}{Refs, always cite article ref and arxiv number}
    \item \textcolor{red}{There are very important references in Alessandra's \cite{buonanno07}.}
    \item \textcolor{red}{See Refs. from T. Spieksma thesis}
    \item \textcolor{red}{Hyperlinks in foot notes, to save things like $x^{i8}\rightarrow x^{i[8]}$.}
    \item \textcolor{red}{non-linearities or nonlinearities?}
\end{enumerate}

\textcolor{red}{Conventions and notations}
\begin{enumerate}
    \item Organizar .bib que poderei usar sempre na pesquisa	
    \item Relaxed for of Einstein's summation convention for spatial indices 
    \item boldface for three(spatial)-vectors 
    \item metric signature
    \item $d$ and $n$ for spatial and spacetime dimensions.
    \item $c=1$
    \item $G_N$ for the Newtonian constnt of gravity in three dimensions.
    \item see pdf that I wrote a while ago on conventions.
    \item ver convnções e notação de Alessandra em \cite{buonanno07} e de Maggioere em \cite{maggiore1,maggiore2}. 
    \item Add notations for symemtrization.
\end{enumerate}


Talvez incluir continhas simples da far zone que escrevi em latex no overleaf, no capítulo das amplitudes.

General symmetric tensors can be projected into its transverse-traceless component by acting the Lambda tensor $\Lambda_{ij,kl}$ on its spatial components. This tensor is 

